Are LLMs Ready for Real-World Materials Discovery?

Large Language Models (LLMs) create exciting possibilities for powerful language processing tools to accelerate research in materials science. While LLMs have great potential to accelerate materials understanding and discovery, they currently fall short in being practical materials science tools. In this position paper, we show relevant failure cases of LLMs in materials science that reveal current limitations of LLMs related to comprehending and reasoning over complex, interconnected materials science knowledge. Given those shortcomings, we outline a framework for developing Materials Science LLMs (MatSci-LLMs) that are grounded in materials science knowledge and hypothesis generation followed by hypothesis testing. The path to attaining performant MatSci-LLMs rests in large part on building high-quality, multi-modal datasets sourced from scientific literature where various information extraction challenges persist. As such, we describe key materials science information extraction challenges which need to be overcome in order to build large-scale, multi-modal datasets that capture valuable materials science knowledge. Finally, we outline a roadmap for applying future MatSci-LLMs for real-world materials discovery via: 1. Automated Knowledge Base Generation; 2. Automated In-Silico Material Design; and 3. MatSci-LLM Integrated Self-Driving Materials Laboratories.

==> 1_intro.tex <==
\section{Introduction}

The advent of large language models (LLMs) has started to reshape many technology development efforts and research roadmaps. Apart from significantly impacting the space of natural language processing, LLMs have had a significant impact on many related fields, such as computer vision with text-to-image generators \citep{zhang2023text}, and have sparked the creation of efforts to integrate their capabilities into diverse industries. Examples of these efforts include task automation in healthcare \citep{he2023survey}, legal \citep{dahl2024large}, finance \citep{wu2023bloomberggpt}, software engineering \citep{fan2023large} and multiple scientific fields. The successful application of LLMs to materials science (MatSci) has the potential to transform the field by accelerating the discovery, synthesis, and analysis of new materials that can address some of today's complex societal-scale challenges, such as climate change, energy security, sustainable agriculture and manufacturing, personalized medical devices, and access to more powerful computing systems. 
% \rev{Among these, materials is a field that has received relatively less attention.} %Materials form the cornerstone in the advancement of human civilization as reflected by several human civilizations named after the major materials used during the period, such as, iron, bronze, etc.} 
While recent research work has seen increased adoption of LLMs in adjacent scientific fields, such as chemistry \citep{jablonka202314} and diverse areas of biology \citep{lin2023evolutionary, pmlr-v162-hsu22a, xu2023protst, cui2023scGPT, dalla2023nucleotide}, the application of LLMs in materials science has been significantly slower. Analyzing the challenges and bottlenecks for the use and development of LLMs tailored to materials is the first step to address this issue. Hence, we aim to analyze the failures of LLMs in materials science and propose requirements for MATerials SCIence LLMs (MatSci-LLMs) along with a roadmap to enable the impactful application of MatSci-LLMs for furthering the field of materials.
% %\vspace{-0.3cm}
% \subsection{MatSci-LLM Requirements}
% %\vspace{-0.1cm}

Material science is a highly interdisciplinary field -- the first scientific branch that emerged out of the fusion of different branches (physics, chemistry, mechanical engineering, and metallurgy) rather than a division -- that studies how the interaction of atomic matter affects the properties and behavior of materials systems across diverse sets of conditions. The broad scope of materials systems encompasses multiple physical scales ranging from nanostructures with a small number of atoms which are used in modern computing devices, to continuum materials, such as metals and cement, that make up modern infrastructure like roads, bridges and buildings. Moreover, the wide range of materials applications can range from electronic materials (e.g., transistors, batteries), to chemical materials (e.g., polymers) to biological materials (e.g., medical implants), each of which has very different requirements and application environments. As such, MatSci often borrows concepts from related scientific fields, including physics, chemistry, and biology, leading to a vast and dynamic body of work covered by the field. This diversity also informs the wide range of tasks that materials scientists perform across different subfields, which further informs the requirements of MatSci-LLMs.

Early work applying text-based methods to materials science largely focused on text-and-data mining. While much progress has been made to enable data mining, many of the challenges data-mining identified in early work by \citet{kononova2021opportunities} remain. One particularly common task for early text-mining methods was mining text to predict synthesis procedures based on peer-reviewed literature \citep{kim2017materials, kim2020inorganic}. While the deployment of targeted text-mining techniques was successful in developing targeted synthesis procedures for a subset of materials systems, the proposed approaches did not provide scalable solutions to a diversity of materials design challenges~\cite{ravinder2021artificial} (see App.~\ref{app.matsyn} for additional discussion). 


In addition to text-mining, early works also focused on classifying the text in materials science publications according to their semantic meaning, which is similar to named-entity-recognition (NER) in traditional language processing \citep{gupta2022matscibert, walker2021impact}. As studied by \citet{song-etal-2023-matsci}, specialized BERT models perform quite well on common NLP tasks for materials science, assuming labeled data exists. This, however, is not scalable given the sparsity of labeled data in materials science. Ensuing information extraction methods, such as ChemDataExtractor \citep{swain2016chemdataextractor} spanned different modalities of data, including scientific text, property data, spectroscopy data, as well as tabular data. Additional efforts were also used to extract information related to images~\cite{venugopal2021looking,zaki2022natural,mukaddem2019imagedataextractor}, which were then used to create either database or to even extract features~\cite{mukaddem2019imagedataextractor,zaki2023cementron}. LLMs have leapfrogged prior machine learning approaches for various text-based MatSci tasks, including information extraction and search. While specialized methods continue to improve the performance of data extraction for applicable modalities in materials science \citep{gupta-etal-2023-discomat}, the advent of LLMs has led to a more unified and reliable way to arrive at reliable information extraction \citep{dagdelen2024structured}. As described in \citet{dagdelen2024structured} and in \Cref{sec:corpus}, in-context learning abilities of modern LLMs are a powerful tool to accelerate the abilities to process and extract information in materials science text. While further research is needed to improve such methods, they represent significant progress that enables new research opportunities discussed in this paper.

In this perspective, we start with an overview of the requirements of a MatSci-LLM. Following this, we discuss the failure cases of LLMs in meeting those requirements and the need for further benchmarking datasets. Next, we discuss the challenges in the development of a MatSci-LLM. This section also presents some of the interesting machine learning challenges involved in the process of building a MatSci-LLM that can be applied to several other domains as well. Concretely, the development of MatSci-LLMs requires high-quality, multi-modal datasets that are curated with the help of domain experts. Moreover, dataset curation also involves a set of unique, on-trivial challenges to potentially unlock the ground-breaking capabilities of MatSci-LLMs. These challenges, amongst others, include linking information across multiple documents referenced via citations, as well as managing diverse ways of expressing important procedures and concepts. To bridge these gaps, we propose a roadmap for MatSci-LLMs, which we hope will enable a coordinated community research effort to address these interwoven challenges. Finally, we discuss the broader implications of MatSci-LLMs and discuss how they could help in addressing some of the sustainable development goals.

\section{Requirements of a MatSci-LLM}
\begin{figure*}[h]
    %\vspace{-0.2cm}
    \centering
    \includegraphics[width=\textwidth]{icml2024/figures/matsci-llm-intro-3.png}
    %\vspace{-0.4cm}
    \caption{Overview of MatSci-LLM requirements related to knowledge acquisition and science acceleration. MatSci-LLMs require knowledge contained across multiple documents along multiple data modalities. Pertinent materials science knowledge includes understanding materials structure, properties and behavior covering diverse conditions, as well as materials synthesis and analysis procedures based on experimental descriptions. To effectively accelerate science, MatSci-LLMs should interact with human scientists as robust question-answering system and act as grounded hypothesis generators that augment a scientist's knowledge. Additionally, MatSci-LLMs should provide executable procedures for real-world experiments through machine-machine and human-machine interfaces.   }
    \label{fig:mat-sci-lllm-req}
    %\vspace{-0.55cm}
\end{figure*}
To evaluate the performance of the LLM for materials science, it is essential to identify the requirements a MatSci LLM needs to satisfy. Given the diversity of MatSci knowledge and its associated technical tasks, we propose that  MatSci-LLM should meet the following requirements, shown in \Cref{fig:mat-sci-lllm-req}, namely, \emph{Domain Knowledge \& Grounded Reasoning:} MatSci-LLMs should have an understanding of MatSci as a subject area to provide useful information to material scientists and be able to reason over core MatSci principles; and \emph{Augmenting Materials Scientists: } MatSci-LLMs should have the ability to perform useful tasks to accelerate materials science research that augments the work of materials scientists in reliable and interpretable manner. These aspects are discussed in detail below.

\textbf{Domain Knowledge \& Grounded Reasoning:} 
% \rev{Earlier efforts on MatSci information extraction relied on rule-based (e.g. regex) approaches and domain-specific training. These approaches, however, could rarely scale beyond the specific materials family studied.} 
Recent research efforts have yielded progress towards infusing MatSci domain knowledge into LLMs to solve text-based tasks. Early work, such as \citet{walker2021impact, gupta2022matscibert, huang2022batterybert} focused on training BERT \citep{devlin-etal-2019-bert} architecture on domain-specific text corpora relevant to MatSci. A detailed analysis of these and other scientific language models by \citet{song-etal-2023-matsci} revealed that domain-specific pretraining did infuse the language models with relevant materials knowledge showing the importance of building high-quality MatSci language datasets. Recent works by \citet{song2023honeybee} and \citet{xie2023darwin} showed that instruction fine-tuning leveraging commercial scale LLMs can further improve performance on MatSci language tasks. While this suggests that practical MatSci knowledge can be extracted from today's commercial LLMs (e.g., GPT-3.5, Claude and GPT-4) their understanding of MatSci remains incomplete as shown by \citet{zaki2024mascqa}. As we discuss in \Cref{sec:failures}, grounded reasoning over materials science principles remains a challenge.

\textbf{Augmenting Materials Scientists:} Research work in this direction has been primarily limited to adjacent domains, in particular chemistry. \citet{jablonka202314} showed different applications of LLMs across diverse chemistry tasks, and \citet{bran2023chemcrow} and \citet{boiko2023autonomous} provided examples of how a tool-augmented GPT-4 can perform real-world experimental planning and execution based on user queries. While such works show great relevance to MatSci, they are incomplete in addressing the vast diversity of knowledge and scientific tasks in MatSci, thereby falling short on the criteria needed to be considered MatSci-LLMs. One concrete difference between chemistry LLMs and MatSci-LLMs, for example, is the fact that IUPAC names in chemistry make the identification and tracking of molecular structures significantly easier. As discussed in \Cref{sec:domain-specific-llm}, the materials domain contains much greater diversity including periodic crystal structures, surfaces, nanostructures, metals and alloys, and disordered materials like glasses, limiting the degree of systematization that can be achieved for indexing these materials with natural language.

%%\vspace{-0.4cm}
%\subsection{What is needed for MatSci LLMs?}
% %\vspace{-0.2cm}

    % \textcolor{red}{can add the code based work from Buehler and other here}

% \section{Related Work \& Current SOTA}

% Talk about LLMs in other disciplines and what they can do - emphasis on the co-scientist work

% \textcolor{blue}{
% Introduce the current state-of-the-art and remaining challenges:
% \begin{itemize}
%     \item Motivate why materials is an important domain (PFAS, energy, etc) - argue that LLM real world deployment for practical applications can be motivated to materials due to its impact; LLMs are not ready for real-world applications (cite co-scientist and chess paper) -> What are the gaps in LLM capabilities?
%     \item Data Extraction from Scientic Papers
%     \item Domain Specific Language in Materials Science
%     \item Explainability, Robustness \& Reliability
%     \item Interfaces to Real-World Actions
%     \item Materials LLM is needed and vanilla LLM are not good enough
%     \item show anecdotal examples of current failures
%     \item highlight the fundamental differences between an LLM (text generation, chatbot, contextual processing, interacting with Internet tools) and a materials LLM (multi-modal scientific data, robust reasoning citing supporting evidence, interacting with real-world tools)
%     \item LLMs have been cited as co-scientists \citep{boiko2023autonomous, bran2023chemcrow} - are they really co-scientists? We say that there is still a lot of work to do. It can basically reproduce what is in the literature, but cannot go beyond that.
% \end{itemize}
% }

==> 2_reliability.tex <==
% \section{LLM Challenges for Materials Science}

% While notable progress has been made in infusing materials science knowledge into both commerial and open-source LLMs, there remain significant challenges in creating performant MatSci-LLMs. \Cref{sec:failures} describes some of the failure cases for modern LLMs with a focus on GPT-4, while \Cref{sec:hypothesi} describes some of the desired behavior.
% The aforementioned challenges of integrating LLMs to act as co-scientists for materials science research outline some of the missing capabilities of current LLMs based on some of the unique challenges of the materials science domain. In addition to being able to resolve domain-specific problems in materials science, LLMs also require greater reliability, robustness and interpretability to become effective tools for significantly accelerate materials science research. 

%\textcolor{red}{
%\subsection{Example of LLM Failures}
%Some examples of LLM failures include: answering scientific questions correctly, understanding limitations of current knowledge with supporting evidence that scientists can use to inform their processes, processing multi-modal scientific data. GPT-4 gets too much math and crystal structure questions wrong in our examples.
%\vspace{-0.4cm}
\section{Failure Cases of LLMs in MatSci} \label{sec:failures}
%\vspace{-0.1cm}
While recent work has shown great promise in applying LLMs to materials science and adjacent fields, it is important to understand the limitations of LLMs on a broad set of challenges in the MatSci domain. To this extent, several efforts have focused on tasks related to question-answering, code writing, named-entity recognition, abstract classification, and composition extraction from tables in materials literature \citep{zaki2024mascqa, gupta-etal-2023-discomat, song2023honeybee, song-etal-2023-matsci}. Here, we outline some of the failure cases demonstrating the need to develop robust MatSci-LLMs before deploying them for practical applications.

Proficient LLMs such as GPT-4 \citep{achiam2023gpt} and LLaMA-2 \citep{touvron2023llama} are trained on vast corpora of publicly available text data \citep{together2023redpajama}. Accordingly, commercial LLMs should have had some reasonable exposure to the MatSci domain based on Wikipedia and other public domain information on MatSci. To evaluate the MatSci domain knowledge of LLMs, \citet{zaki2024mascqa} curated a dataset of 650 questions requiring undergraduate-level knowledge to answer them. The analysis of the responses from LLMs revealed that GPT-4 with chain-of-thought (CoT) \citep{wei2022chain} reasoning performed the best with a score of 62\% accuracy. Interestingly, GPT4-CoT performed the worst in numerical-type questions with a score of only 39\%. This suggests that present LLMs perform poorly in identifying the correct equations, grounding the context by substituting appropriate numerical values, and subsequently solving the original question. Moreover, a comparison of the performance of LLMs with human performance in the same exam revealed that GPT4-CoT, while outperforming other baselines, consistently obtained only 50\% of the top-performing humans and ultimately never cleared the cutoff to pass the exams. 

A task where LLMs are known to perform well is code generation \citep{chen2021evaluating, lai2023ds, zan2023large}. While code generation for chemistry tasks has yielded mostly promising results as detailed in \citet{white2023assessment}, \citet{zaki2024mascqa} evaluated the performance of LLMs on code generation tasks as well and found that GPT-4 exhibited an accuracy of only 71\% even in code writing tasks related to MatSci. A careful analysis of the questions and code-writing tasks where GPT4-CoT performed poorly reveals two salient conclusions: (i) LLMs have difficulty in solving complex numerical problems, not just because of the complex arithmetic (which could potentially be solved by translating the numerical question into code \citep{wu2023empirical}), but because of their inability to ground the available data in the given equation. This includes wrong substitution, incorrect conversion of units, and missing constants while converting units (e.g., taking into account the speed of light, Avagadro number, etc.). (ii) LLMs have difficulty in understanding the information related to 3D structure. Specifically, the crystal structures and the symmetries associated with materials are misinterpreted leading to incorrect conclusions. \citet{zaki2024mascqa} observed these errors consistently in both code generation tasks and question-answering tasks for multiple LLMs. 

To elucidate current LLM failure cases in MatSci, consider the question below. \textit{``The materials belonging to which one of the following crystal classes would be both piezoelectric and ferroelectric: (A) 222 (B) 4mm (C) -1 (D) 2/m''.} Here, while (B) 4mm is the correct answer, GPT4-CoT suggests 2/m as the correct answer with the reasoning that \textit{``(D) 2/m: This crystal class does not have a center of symmetry, which means it can be piezoelectric. Additionally, it is a polar crystal class, making it able to be ferroelectric as well.''}. However, this reasoning is incorrect---2/m is centrosymmetric, and hence is not a polar crystal. Answering this question requires the knowledge of crystal structures, which needs to be grounded on the concept of the polarity of atoms based on the crystal structure. Although the LLM understands this requirement, it performs poor reasoning and inference, potentially due to the lack of such data during training. Another example worth noting is the following question. \textit{``The Miller indices of the first three Bragg peaks in the X-ray diffraction pattern obtained from a polycrystalline iron sample at room temperature are (A) (111), (200), (220) (B) (100), (110), (111) (C) (100), (110), (200) (D) (110), (200), (220)''}. While the correct answer is (D), GPT4-CoT suggests (C) as the answer, based on the reasoning that \textit{``systematically listing all possible combinations of h, k, and l, and identifying those that satisfy the BCC selection rule (h + k + l = even), we get the following allowable Miller indices as: (100), (110), and (200)''}. However, this is contradictory as for the first Miller index (100) in the list, h + k + l = 1 + 0 + 0 = 1, which is odd and not even. Accordingly, while the understanding that the BCC selection rule requires (h + k + l) should be even is correct, the LLM was unable to ground this concept correctly and suggest the correct Miller indices. Ten such examples are listed in Appendix~\ref{App:mistakes}, where we provide the question, the answer, and the reasoning provided by GPT-4, along with the correct solution. We observe consistent mistakes made by GPT-4 in numerical errors and reasoning inconsistencies both in conceptual MatSci questions and in MatSci code generation tasks. These observations strongly suggest that LLMs need to be exposed to more domain-specific information and develop greater reasoning capabilities for them to be usable for any real-world application in this domain.

LLM reasoning difficulties extend beyond the MatSci domain, including in general language tasks \citep{behnamghader-etal-2023-retriever}.
% The difficulties in LLM reasoning have been documented beyond the MatSci domain .
Given the great importance of reasoning abilities to formulate and test scientific hypotheses, this remains a major gap in the development of MatSci-LLMs which also has implications for the broader LLM community. While LLMs have shown promise in solving concrete planning tasks, such as retrosynthesis planning \citep{boiko2023autonomous,bran2023chemcrow}, and executing code-based functions as part of a greater workflow \citep{buehler2023generative,yoshikawa2023large}, LLMs still rely on human intervention and correction in many cases. In addition to greater robustness, future LLMs can also benefit from greater interpretability to accelerate hypothesis testing and enable scientists to better understand the various aspects of the system they are interested in. This is especially important in MatSci where many experimental procedures can expose valuable information about the underlying material properties and behavior under diverse settings, which in turn can inform a broader understanding of fundamental physical and chemical relationships of the underlying material system. 

To fully unlock the power of LLMs for materials discovery, further progress is needed along the following directions.\\
\textbf{1. Hypothesis Generation Grounded on MatSci Knowledge: } MatSci-LLMs require an understanding of diverse MatSci knowledge and the ability to reason over core domain principles. This will enable MatSci-LLMs to answer queries of domain-specific questions and generate useful hypotheses that can be verified with real-world experiments. Modern LLMs struggle to provide well-reasoned answers that reference relevant supporting evidence for in-depth questions. While ongoing progress highlights the capability of modern LLMs to provide relevant MatSci knowledge \citep{song2023honeybee}, clear gaps remain \citep{zaki2024mascqa}.\\
\textbf{2. Multi-Modal MatSci Datasets:} To enable MatSci-LLMs to capture the true extent of human knowledge of MatSci, we require large-scale, high-quality, multi-modal datasets based primarily on peer-reviewed MatSci publications. Much of the knowledge in the MatSci literature is contained in tables, figures, and other modalities that express important material properties and behavior in addition to the physical and chemical relationships that underlie them. Additionally, modern LLMs still struggle to understand domain-specific MatSci language and effectively process MatSci notation, including chemical formulas and mathematical formulas expressed in line with other text.\\ 
\textbf{3. Real-World Materials Design:} Connecting MatSci-LLMs to real-world simulation and experimental tools in creative ways can comprehensively accelerate materials design, synthesis, and analysis by enabling end-to-end automation. As described in \Cref{sec:roadmap}, MatSci-LLMs can provide powerful human-machine and machine-machine interfaces for increased automation in MatSci research, as well as commercial materials production. Recent work in chemistry LLMs \citep{bran2023chemcrow, boiko2023autonomous} has shown promise in deploying tool-augmented LLMs for end-to-end materials design tasks driven by text-based user input.

\begin{table}[ht]
\begin{spacing}{1.0}
\centering
% %%\vspace{-2.5mm}
\begin{adjustbox}{max width=1\linewidth}
\label{tab:matsci-llm-tasks}
    \begin{tabular}{c|c|c}
        \toprule
        \bf{Dataset} & \bf{NLP Tasks} & \bf{References} \\
        \midrule
        {1. Battery Device QA} & In-context Q\&A & \cite{huang2022batterybert}\\
        \midrule
        {2. MaScQA} & Materials Q\&A, Code generation,\\ & Composition extraction & \cite{zaki2024mascqa,gupta-etal-2023-discomat}  \\
        \midrule
        {3. MatSciNLP} & Named entity recognition,  & \cite{song-etal-2023-matsci,gupta2022matscibert} \\ & synthesis action retrieval,  & \cite{jensen2021discovering,kim2020inorganic} \\ & event argument extraction, & \cite{kim2017materials,mysore2019materials} \\ & paragraph classification, \\ & relation extraction, \\ & sentence classification, slot filling \\
        \midrule
        {4. OpticalTable Q\&A} & Table and text-based Q\&A & \cite{zhao2023opticalbert}  \\
        \midrule
        {5. SustainableConcrete} & Text-based Concrete Design & \cite{volker2024llms}  \\
        \bottomrule
    \end{tabular}
\end{adjustbox}
\end{spacing}
\caption{Benchmarking datasets for MatSci-LLM along with the tasks.\label{tab:matscillmbenchmark}}
%%\vspace{-2.5mm}
\end{table}

\textbf{Datasets and benchmarking:} Evaluating the performance of LLMs on these tasks requires several carefully curated datasets and benchmarking frameworks that evaluate the model performance and limitations. Although there are several datasets available as listed in \Cref{tab:matscillmbenchmark}, further work is needed to systemically assess LLMs capabilities related to MatSci. Specifically, there are limited datasets covering only a small aspect of the wide range of topics related to materials. Moreover, there exist no datasets on multi-modal evaluations including text, graphs, figures, tables, audio, and video. On top of that, there are limited datasets on experimental procedures and protocols that could be used to evaluate the knowledge of LLMs related to understanding and executing relevant experimental procedures. It is worth noting that there are increasing research efforts on evaluating the performance of LLMs for chemistry that have led to more advanced datasets, benchmarks, and analysis \citep{mirza2024large}. We believe that similar efforts need to be carried out in the materials science domain as well, including but not limited to the area of composites, metals, alloys, ceramics, glasses, and nanomaterials.
% \subsection{Grounded Reasoning \& Hypothesis Generation} \label{sec:hypothesi}
% Much of the evidence in prior work shows that while LLMs can be useful for a range of practical tasks, sometimes they can fail in unexpected ways \citep{boiko2023autonomous}. While it is not necessary for LLMs to be robust for all tasks and queries to be useful scientific tools, it would be helpful for the types of failures and limitations to become more predictable enabling scientists to apply the LLMs in with greater confidence in settings where they provide reliable performance. While the body of literature on making LLMs more robust in general language settings continues to make rapid progress, future works still remains for better understanding LLMs' reasoning abilities for both retriever-augmented generation (RAG) and non-retriever based LLMs \citep{behnamghader-etal-2023-retriever}. Advances in further understanding reasoning abilities and infusing more structured knowledge into LLMs in general language settings can continue to inform scientific applications of LLMs as limitations become more well-known and mitigation techniques continue to be improved. 


% % \subsubsection{Hypothesis Generation \& Testing}
% One particularly important task for for scientific applications is the ability to formulate hypothesis, define an experimental plan for testing said hypothesis and analyzing the data to understand whether the evidence supports the original hypothesis. Current LLMs often fall short in their ability to both formulate and define a testing plan for a given hypothesis. In order for LLMs to become effective co-scientists, they should be able to productively interact with human scientists to develop procedures for both hypothesis generation and hypothesis testing. Many of the capabilities in scientific application papers today such as \citet{bran2023chemcrow} mainly focus on LLMs' abilities to execute procedures based on faily concrete instructions based on targeted prompts with much work remaining on understanding the braoder scientific capabilities and limitations of LLMs. 

% The context of hypothesis testing also requires a great degree of interpretability, both in developing the experimental procedure and in executing it, so that scientists can understand the various aspects of the system they are interested in. This is especially important in materials science where many experimental procudures can expose valuable information about the underlying material properties and behavior under diverse settings, which in turn can inform broader understanding of fundamental physical and chemical relationships. 

% % \textcolor{blue}{
% The challenges here deal with common issues of LLMs, including:
% \begin{itemize}
%     \item Hallucinations
%     \item Providing reasoning based on explicit and implicit knowledge
%     \item Provide tests and ability and to generate and verify hypotheses
%     \item synthesis case where one needs to retrieve recipes in a reliable manner
%     \item talk about whether RAG ground something on data -> evidence is unclear
%     \item look at these factors from the perspective of what an LLM co-scientist needs -> avoid generic LLM discussion
% \end{itemize}
% }

==> 3_domain_language.tex <==

%\vspace{-0.3cm}
\section{Challenges in the development of MatSci-LLM} \label{sec:domain-specific-llm}
%\vspace{-0.1cm}
The MatSci domain requires great technical depth and breadth due to the field's broad technical scope that interfaces with physics, chemistry, biology, and various engineering disciplines. Hence, MatSci presents unique challenges for knowledge acquisition for domain-specific language models.
% Due to its broad technical scope that interfaces with physics, chemistry, biology and various engineering disciplines, MatSci presents a unique challenge related to understanding given the field's breadth across disciplines and depth in detail and understanding required. 
While some of the challenges, such as domain-specific notations, are unique to MatSci, others have a broad intersection with multiple machine learning fields, such as multi-modal information extraction involving text, images, and video.

\textbf{Domain-Specific Notations:} Unlike IUPAC \citep{hellwich2020brief} nomenclatures in chemistry, there exist no standard notations for MatSci; for instance, NaAlSi$_2$O$_8$, Na$_2$O.Al$_2$O$_3$.2SiO$_2$, SiO$_2$--0.5Na$_2$O--0.5Al$_2$O$_3$ all represent the same material in different contexts. Moreover, several common domain-specific names represent materials, including soda and lime, for Na$_2$CO$_3$ and CaCO$_3$, respectively. Furthermore, some sub-domains, such as cement, employ their own chemical notations that are contradictory with the general chemistry notation; C-S-H represents calcium silicate hydrate in cement chemistry, whereas, in standard chemistry notation, it represents carbon, sulfur, and hydrogen, respectively. Similarly, there are several inconsistent abbreviations used in the literature to refer to properties in MatSci. These abbreviations are sometimes specific to a given document or can also be present in multiple documents. Thus, understanding these notations requires grounding the LLMs in different domains with the right context.
    
\textbf{Incomplete Descriptions:} Research publications regularly refer to previous works in the text to omit specific information. This is exemplified by the sentences such as \textit{``the fracture simulations were carried out using an established methodology as outlined in Griffith et al.''}; a common practice in the MatSci literature. Such approaches are also extremely common when reporting experimental or simulation protocols, material compositions, syntheses, and testing conditions, and optimizing process parameters. The context of the work reported in a manuscript, in this case, is thus grounded in a different manuscript. Moreover, the descriptions can occasionally be highly non-linear while referring to different sources in an extremely complicated manner. Finally, there could be a reference to the manuals of different instruments and material sources, which are described elsewhere. Thus, an LLM needs to procure information across multiple sources and process it together in the proper context to create a sequential description of the process and the related analysis that was carried out.

\textbf{Text-to-Structure:} MatSci employs text to represent several 3D or 2D structures in different ways. For instance, the crystal structures are represented using the Wyckoff positions \citep{aroyo2006bilbao} --4mm in crystallography represents a crystal structure, whereas, in general literature, it might be confused with a distance metric (millimeter). Moreover, crystals are represented using a widely used format known as crystal information file (CIF), which explains the details of the crystal along with the positions of the atoms as shown in \Cref{app.cif} with a CIF of Silicon. Current LLMs are unable to read, interpret, or generate CIF in their entirety, which is a strong limiting factor for novel materials discovery. Similarly, there are several other approaches to represent the 3D structure using text, such as XYZ files or other software-specific files for diverse purposes. As such, the ability of LLMs to understand such files plays a crucial role in the materials domain. Recent work by \citet{gruver2023finetuned} shows that LLMs can generate correct CIF-formatted materials with targeted fine-tuning but fail to provide context describing important details of the CIF file.
    
\textbf{Multi-Modal Information Extraction: Text and Tables:} Pertinent information for materials in peer-reviewed papers are generally represented using multiple modalities, including text, tables, figures, and videos---audio is rarely used, although not absent. Significant progress has been made in effectively extracting tabular information \citep{gupta-etal-2023-discomat,zhao2023opticalbert,zhao2022database} with work still remaining on how to best make use of extracted data to infuse the underlying knowledge of the tables into language models. Extraction can be particularly challenging for property-based data, which often includes numbers that map to various scientific units. A simple exercise on information extraction from tables revealed that GPT-4 was able to extract only $\sim 55\%$ of materials properties from a table \citep{zaki2024mascqa} in contrast to $\sim 73\%$\ by a model trained for the task \citep{gupta-etal-2023-discomat}. This problem is amplified by the fact that more than 80\% of material compositions and properties are reported in tables \citep{hira2023reconstructing}. Finally, in several cases, table information is incomplete, even when read together with the caption. For instance, when reporting the composition of Magnesium alloys, many tables in research papers report the values of all the components other than Magnesium in a given alloy. Thus, the percentage of Magnesium in these alloys needs to be computed as 100-(the sum of reported elements in the tables for a given alloy). Such a task requires grounding the table information along with the text and then performing the necessary arithmetic to obtain the percentage. 

\textbf{Multi-Modal Information Extraction: Text and Figures:}
 Materials are characterized by many experimental methods such as Raman analysis, X-ray diffraction (XRD), X-ray fluorescence, scanning electron micrographs, or atomic force microscopy, the results of which are represented in figures. Such information could include the visual representation captured by the measurement technique, such as an optical micrograph or a plot that summarizes this information, as in the case of XRD patterns. Moreover, this information will be elaborated briefly in the figure caption, followed by a detailed explanation in the text. A sample text from a materials literature could be as follows: \textit{``The XRD patterns shown in Figure XY(a) suggest that the sample is amorphous and does not have any crystalline content. Further, the XRF in Fig. XY(b) reveals the presence of clustering of Calcium instead of a uniform distribution''}. In this particular case, the text and figure need to be interpreted together. Moreover, the specific aspects of the image that allow one to interpret it, such as the clustering of calcium or the specific feature of the XRD patterns, allow a researcher to identify that the material is amorphous and is not labeled. In order for the LLM to learn these aspects, a large number of images and aligned text are needed for joint training.

\textbf{Multi-Modal Information Extraction: Text, Figures, Tables, and Videos:} Additional modalities of presenting relevant information involve a combination of text, figures, and tables. In such cases, the information from the table should be read along with the figures while grounding the reasoning in the context of the manuscript, all of which further compound the cumulative importance of multi-modal information extraction. Occasionally, additional modalities, such as audio-visual files, are used to demonstrate material response. This includes material failure modes illustrating cracks, crystal growth, thermal response, the response of actuators, and simulations, amongst others. In this case, there are additional challenges that require the training of LLMs to properly link the information in video, figures, text, and tables. These are open problems for which the community may need to develop novel methods and architectures. While these challenges are far from exhaustive, we note that the tasks mentioned here reveal novel domain-specific problems whose solutions can have a potentially strong impact on other scientific and machine learning domains as well.
% \textcolor{red}{intersection with other domains in vision and science is relevant here}
% %\vspace{-0.3cm}

\textbf{Context Across Multiple Documents \& Sources:}
% %\vspace{-0.1cm}
Most of the information generated through scientific inquiry is documented and communicated through natural language in peer-reviewed publications. Understanding this text -- and potentially extracting the information -- presents several unique challenges distinct from other domains \citep{hira2023reconstructing}. One of the major challenges in this regard includes understanding the importance of context across multiple documents and sources of information. As highlighted above, this is additionally complicated by the fact that a given material can have multiple correct names and designations, meaning that important information can be contained across all of the names for a given material. 
% This is a significant difference from adjacent fields, such as chemistry, which have standardized naming conventions like IUPAC nomenclature that designate concrete compounds. The IUPAC naming convention makes it easier for data to be organized with a unique identifier which can then be effectively processed by LLMs to understand relevant information within a single, and potentially multiple documents. 
Having unique IUPAC-style naming conventions can accelerate the deployment of LLMs as observed in chemistry \citep{jablonka202314}, yet this is often not sufficient to capture all the relevant details needed to fully understand materials properties and synthesis leading to the development of additional data initiatives to fill that gap \citep{kearnes2021open, mercado2023data}. Hence, while proposing an IUPAC-style naming convention might seem like a natural solution to aid the deployment of LLMs in MatSci, many proposals of such conventions have previously fallen short, given the vast diversity of the field.
% %\vspace{-0.3cm}

\textbf{Diverse Experimental and Simulation Procedures:} \label{app.matsyn}
% %\vspace{-0.1cm}
While understanding context is the first step toward automated discovery, the next natural step is to identify the appropriate experimental or simulation protocols relevant to the context. There is a multitude of experimental and simulation procedures that can be used to evaluate the same objective. As such, understanding them and choosing the relevant one or a set of relevant experiments is a challenging task, which requires domain-specific information and reasoning. Early works have shown some promise in providing useful tools for creating synthesis procedures of specific materials \citep{olivetti2020data, jensen2021discovering}, but much work remains in effectively deploying LLMs for these tasks. 
% In addition to having to resolve context across multiple documents due to the fact that complimentary information for synthesis procedures can be provided by multiple sources, 
Additionally, understanding experimental MatSci procedures provides additional challenges given the diversity of synthesis, characterization techniques across data modalities (e.g., phase identification using X-ray diffraction, spectroscopic techniques), and processing conditions that can be observed across materials design use cases even within similar materials classes. %(\rev{see App.~\ref{app.matsyn} for a detailed discussion}).
% \rev{Materials characterization experiments also require MatSci-LLMs to effectively manage diverse data modalities (e.g., phase identification using X-ray diffraction, spectroscopic techniques)}. 
Similarly, effective \textit{insilico} design and filtering of materials requires accurate simulations, and the inability to generate the correct codes grounded in the context can make this task challenging. This is exemplified by the mistakes in the code generation tasks where the LLMs are unable to either ground the concept correctly or the generated code exhibits numerical errors. Thus, it is imperative that large amounts of curated and complete data associated with simulation and experimental procedures are used to train effective MatSci-LLMs. %One such example is the difference of gas-phased processing and liquid-phase processing for the same material (\textcolor{red}{need an example here)} systems which has vastly different equipment requirements and processing conditions required. 

It is worth noting that understanding materials synthesis and characterizing them is far from trivial given the cast diversity of procedures, many of which can exist even among the same family of materials. Modern materials systems range from metals, ceramics, semiconductors, glasses, and polymers to composites, nanomaterials, alloys, and biomaterials to name a few. Furthermore, many materials exist in liquid, solid (both amorphous and crystalline), or gaseous phases. Composites, which involve combinations of multiple materials, often contain multiple phases in a single system such as a gel, which is a liquid in solid, or a colloid, which is a solid in liquid. 
The synthesis procedures relevant for these diverse arrays of materials accordingly vary greatly and include diverse methods such as melt-quenching, sintering, annealing, sol-gel process to name a few. Following synthesis, characterizing the synthesized materials is also a noteworthy challenge where each technique needs to be mapped to the given system and property of interest. To further complicate matters, the same property measured by different techniques can lead to different results.
% For instance, for an amorphous material, XRD along with ICP-MS could be used to ensure the amorphous nature and the precise composition. on the contrary, for a liquid system, this might not be appropriate. 
% Further, the characterization technique to be used for the material also depends on the nature of the property of interest and the length scale of interest. 
For instance, hardness measured by common techniques including nanoindentation, microindentation, atomic force microscopy, a picoindenter~\cite{gouldstone2007indentation}, or a scratch test~\cite{kasimuthumaniyan2021towards}, all can yield significantly different results. Altogether, the diversity in these approaches suggest that synthesis and characterization procedures must be customized for each individual material system. As such, this type of information is important to the MatSci-LLM to understand have available in order for it to suggest the appropriate experimental technique and enable its execution.

Addressing this challenge requires a comprehensive database of synthesis and characterization data of materials. Early work, such as  \href{https://www.synthesisproject.org/publications}{the synthesis project} \citep{kim2017materials,kim2020inorganic} have started to collect such data for a subset of modern materials. Additionally, past research efforts have focused on extracting information related to processing and testing conditions of materials \citep{mysore2019materials,venugopal2021looking,zaki2022extracting}, which are acutely valuable for building comprehensive databases. 
% Recently, efforts have also been employed to use the textual data for predicting the corrosion of alloys by incorporating the testing conditions \citep{sasidhar2023enhancing}. 
% These are some of the promising directions to pursue to have an extensive KN system for the synthesis and characterization of materials. 
Many of the aforementioned approaches employed classical natural language processing techniques which can benefit from the enhanced capabilities of modern LLMs. 
% Combining these datasets along with LLMs could further enhance the usability of these approaches.

% \textcolor{blue}{
% The challengs in domain-specific materials language:
% \begin{itemize}
%     \item the strong importance of context for materials names and designation (examples of different names for different materials)
%     \item important context can be written across different that use different names for the same materials and potentially even the same property
%     \item the context of procedures and what is needed -> introduce how LLMs can make MatSci more reproducible if used properly
%     \item chemical notations, abbreviation, jargon, equations and understanding relationships (mention reasoning and logic synthesis progress here)
%     \item UIPAC is chemistry and non-UIPAC is materials -> no standard notation for materials leading to a greater challenge. 
%     \item Materials synthesis protocols can be diverse and very sensitive -> non-linaer synthesis and testing protocols; compare to serial procedures that are often found in chemistry
% \end{itemize}
% }

==> 4_extraction.tex <==
% \section{Roadmap for MatSci-LLMs}
%\vspace{-0.2cm}
\section{Multi-Modal MatSci Corpus Building} \label{sec:corpus}
%\vspace{-0.1cm}
The performance of a language model heavily depends on the quality of the dataset on which they are trained on. Thus, dataset creation remains an integral part in enabling progress across various deep learning subfields, including computer vision, graph learning, as well as natural language in both general and scientific domains. 
% MatSci has several domain-specific variations in terms of text, and recent developments in multi-modal language models motivate the development of datasets that align the additional modalities such as figures, tables, and images. 
Given the vast amount of MatSci information expressed in diverse modalities, multi-modal language models would unlock significantly more powerful capabilities for scientific language modeling.

The gold standard data for training these LLMs for MatSci is mostly contained in peer-reviewed publications at established editorials, such as the family of journals at Elsevier, Royal Society, American Society, and Springer Nature amongst others. Unfortunately, much of the content of peer-reviewed publications at established journals remains inaccessible beyond paywalls limiting public access, which makes it difficult to access these valuable text data. Accordingly, it is unlikely that any general-purpose language models, such as GPT-4 or LLaMa, have had access to this data, which likely contributes to their poor performance on MatSci tasks highlighted in \Cref{sec:failures}. While there have been promising developments in making scientific text data available via open access through various preprint servers and portals like Semantic Scholar, text data obtained from such sources often requires extensive cleaning and preparation processes before becoming useful for training scientific LLMs \citep{lo-wang-2020-s2orc}. Research work in making text data more accessible has already produced meaningful results in making language model training and evaluation more successful \citep{song-etal-2023-matsci, song2023honeybee}. However, curating such data on which an LLM can be trained requires addressing additional data-related challenges described below.
% . Some of these challenges are outlined below.

\textbf{1. Data Availability:} 
% \rev{First requirement for training a domain specific LLM is to use high-quality text data.} 
While families of journals such as Elsevier and Springer provide text and data-mining APIs based on paid subscriptions, machine-readable formats such as xml files are available only for manuscripts published in the 21$^\textrm{st}$ century. Our analysis of MatSci-related articles in Springer and Elsevier journals revealed that $\sim$ 6 million peer-reviewed articles with a total of $\sim$ 20 billion words are available in a machine-readable format through institutional subscriptions (see \Cref{app.list}). While this corpus is significantly smaller compared to general language LLMs, the quality and domain relevance is significantly higher. 
Nevertheless, almost all the publications from the 20$^{\mathrm{th}}$ century or earlier are only available as PDFs or scanned files of the hardcopy publication which are not easily machine-readable. Thus, a vast amount of data representing the cumulative scientific endeavor before the 21st century is not available for LLM training. Additionally, many other families of peer-reviewed journals do not either allow text and data mining or have a framework to support it. Data sourced from preprint servers, such as arXiv, often require extensive cleaning to make them amendable to LLM training.
% Moreover, this dataset for pretraining does not require any annotations assuming that we employ self-supervised learning pioneered by LLMs.}\\

\textbf{2. Large-Scale Description \& Annotation:} %When data is obtained from multiple sources and in multiple modalities, such as tables, text, images, videos, and codes, appropriate descriptions that align the various modalities are required to enable effective training.
While pretraining does not require annotations, several downstream tasks require high-quality annotations for finetuning the model or employing it using in-context or few-shot learning. This is particularly important when data is obtained from multiple sources and in multiple modalities, such as tables, text, images, videos, and codes. For instance, a CIF document of Silicon should have a detailed description of what information is contained in the file so that the LLM can learn to interpret the information in the CIF in addition to understanding its format. However, such large-scale annotations are currently unavailable and would require input from domain experts for them to be reliable. Given these challenges, to ensure scalable dataset generation, we propose: 
% (a) distant supervision, (b) using general purpose language models based on in-context learning, and (c) domain specific regex.(a) 
\textbf{a. Distant Supervision:} Here, sparse supervision signals are used to alleviate the amount of high-quality annotations required. This has shown promise in data extraction \citep{gupta-etal-2023-discomat} and can be applied along with existing materials databases, such as the Cambridge Structure Database \citep{groom2016cambridge}.
% , and  \href{https://www.newglass.jp/interglad_n/index_e.html}{Interglad}.\\
\textbf{b. In-Context Learning:} General purpose LLMs, such as GPT4, exhibit excellent in-context learning capabilities. Thus, prompt engineering along with in-context learning can be used to generate high-quality training data. \citet{song2023honeybee} demonstrated this approach for instructions-based finetuning of an LLM for materials science tasks. We provide several examples of composition extractions detailed in \Cref{app.gpt4_comp}, which show some of the capabilities and gaps of in-context learning for GPT-4. 
% as follows. 
% ``Extract all the compositions from the following expression. (70 - x)TeO2 + 15B2O3 + 15P2O5 + xLi2O, where x = 5, 10, 15, 20, 25 and 30 mol\%'': GPT4 was able to extract the compositions. 
% ``Extract all the compositions from the following expression. Glasses with composition in mol\%: 51ZrF4, 16BaF2, 5LaF3, 3AlF3, 20LiF, 5PbF2 have been prepared. +xErF$_3$ from 0.01 to 11 mol\%'': GPT4 was partially successful as the exact composition of dopant was not present in the sentence.
% ``Extract all the compositions from the following expression. Lithium disilicate glass was prepared in 30 g quantity by heating stoichiometric homogeneous mixtures of lithium carbonate (99.0\%), Synth, and silica (99.9999\%), Santa Rosa, for 4 h at 1500°C in a platinum crucible.'':GPT-4 was able to identify the constitutents but was unable to extract exact composition percentages for the same. Detailed experiments and output from the GPT4 are now included in the App.~\ref{app.gpt4_comp}. 
% This approach has also been demonstrated in instruction-based fine-tuning of LLMs for MatSci~\cite{song2023honeybee}.\\
\textbf{c. Domain-Specific Regex} can also be very useful in developing high-quality training data. Robocrystallographer \citep{ganose2019robocrystallographer}, for example, is a regex-based approach that can produce a textual description for a CIF file. Similarly, ChemDataExtractor \citep{swain2016chemdataextractor} employs a regex-based approach for chemical data extraction. Regex tools, along with LLMs and distant supervision, comprise promising methods for scalable data generation and materials design challenges discussed in \Cref{tab:matsci-llm-tasks}.

\textbf{3. Linking Multiple Entities:} While obtaining data on multiple entities is possible, linking them appropriately so they can be read together with relevant context is a non-trivial task. For instance, the description of a figure or a table in a manuscript could be spread across multiple paragraphs and even the supplementary material. This is in contrast to standard machine learning approaches where a figure and description are given together while training. Thus, developing a dataset that links multiple entities appropriately and employing an appropriate training scheme that respects the dataset and the context remains an open challenge for the research community.

\textbf{4. Handling External References:} Another major challenge while curating a dataset based on peer-reviewed publications relates to the use of external references. In a manuscript, references to multiple documents will be made to either support the claims made in the current work and thereby base the manuscript to be read in the context of the referred work. In other words, information in the present manuscript is grounded on the claims or observations in the referenced manuscript, which in turn is grounded in its own references. Dataset and training schemes developed to train a MatSci-LLM should respect this fact to reduce hallucinations and provide well-reasoned, executable hypotheses. It is also worth noting that several LLMs often hallucinate when asked for references. Furthermore, when asked to generate a text in the form of a scientific manuscript, these LLMs generate fictitious references which are arbitrarily written to fit sentences generated in the process. This motivates the need to appropriately account for external references in the training data.

Altogether, these challenges suggest that the development of a dataset for MatSci-LLMs requires close collaboration between multiple entities, including publishers, government, industry and academia. While development of high-quality datasets are indeed challenging, employing some of the aforementioned approaches along with the development of new methods for managing sparse datasets can spark research for novel solutions that effectively manage data sparsity in the MatSci domain. Moreover, MatSci-LLMs warrant machine learning solutions for several new challenges such as: (i) handling old and non-machine readable data through computer vision techniques that can convert the scanned documents to text respecting the original formats, and (ii) novel machine learning methods that can handle external references and multi-modal data that are linked together across different contexts. Such solutions could have implications beyond the MatSci domain, such as analyzing old documents relevant to the history, law, and finance.
% \textcolor{black}{
% The main challenges in data extraction are:
% \begin{itemize}
%     \item paywalled journal content that could be easily accessible - outline all available sources for MatSci langauge data today including \citep{song-etal-2023-matsci, song2023honeybee, lo-wang-2020-s2orc, zaki2024mascqa} and the Chem-NLP project from Europe (explain difference between chemistry and MatSci)
%     \item challenges in extraction of text and non-text data (text from PDF, Figures, Tables) and what the state-of-the-art in each of them is
%     \item what is missing (e.g. annotated images of SEM or other data that identify important things in images or spectra) 
% \end{itemize}
% }

==> 5_interfaces.tex <==
% \subsection{Applying MatSci-LLMs for Real-World Materials Design}
%%\vspace{-0.4cm}
\section{Roadmap for MatSci-LLMs} \label{sec:roadmap}
%%\vspace{-0.2cm}
% One of the most exciting opportunities is the application of MatSci-LLMs for end-to-end automation of materials design. Moreoever, automated materials design can in turn accelerate research in understanding the diverse scientific complexities involved in MatSci. 
\Cref{fig:mat-sci-lllm-roadmap} shows our proposed outline of an end-to-end materials discovery framework with MatSci-LLM at the core. Each part of the roadmap contains diverse research opportunities building towards a performant MatSci-LLMs. Furthermore, \Cref{tab:matscillmtasks} outlines some of the recent attempts to address these challenges. Now, we discuss these set of tasks for MatSci-LLMs spanning the six steps specified in the roadmap in \Cref{fig:mat-sci-lllm-roadmap}. 


\begin{figure}[h!]
    %%\vspace{-0.3cm}
    \centering
    \includegraphics[width=0.8\textwidth]{icml2024/figures/matsci-llm-roadmap-3.png}
    %%\vspace{-0.5cm}
    \caption{Roadmap of a Mat-Sci LLM based materials discovery cycle. The cycle starts with materials query from a researcher that specifies desired properties or an application. The MatSci-LLM then draws from external and internal knowledge bases to generate a materials design hypothesis which is evaluated in-silico. Next, the MatSci-LLM ingests the in-silico results and prepares an experimental plan to synthesize and characterize the material, after which the MatSci-LLM interfaces with the relevant machines to execute the experimental workflow. The final result is then shown to the user for evaluation and feedback. Each stage can interact with another for refinement and improvement by the MatSci-LLM. }
    \label{fig:mat-sci-lllm-roadmap}
    %%\vspace{-0.3cm}
\end{figure}

% The roadmap is broken in six different steps, each of which includes diverse research opportunities. These opportunities can improve the capabilities for each individually while also connecting the various pieces needed to unblock the potential benefits of MatSci-LLMs. 

\begin{table}[ht]
\begin{spacing}{1.0}
\centering
% %%\vspace{-2.5mm}
\begin{adjustbox}{max width=1\linewidth}
\label{tab:matsci-llm-tasks}
    \begin{tabular}{l|c|c}
        \toprule
        \bf{Roadmap Step} & \bf{MatSci-LLM Tasks} & \bf{References} \\
        \midrule
        \multirow{2}{*}{1. Materials Query} & \makecell{Prompting} &  \makecell{ } \\
        \cmidrule{2-3}
         & \makecell{Human-Machine Interfaces} &  \makecell{ \citep{vasudevan2022discovering}} \\
        
        \midrule
        \multirow{2}{*}{2. Data Retrieval} & \makecell{RAG} &  \makecell{} \\
        \cmidrule{2-3}
         & \makecell{Externalizing Knowledge} &  \makecell{ \citep{buehler2024mechgpt, venugopal2024matkg}   } \\

        \midrule
        \multirow{2}{*}{3. Materials Design} & \makecell{Text-Based Design } &  \makecell{ \citep{gruver2023finetuned, flam2023language}} \\
        \cmidrule{2-3}
         & \makecell{Generative Model Tools} &  \makecell{ \citep{zeni2023mattergen, govindarajan2023learning}   } \\
        
        \midrule
        \multirow{2}{*}{4. Insilico Evaluation} & \makecell{Predictive Modeling} &  \makecell{ \citep{rubungo2023llm, jablonka202314} } \\
        \cmidrule{2-3}
         & \makecell{Code Generation} &  \makecell{ \citep{zaki2024mascqa}  } \\
        
        \midrule
        \multirow{2}{*}{5. Experimental Planning} & \makecell{Task Automation } &  \makecell{ \citep{bran2023chemcrow, boiko2023autonomous} } \\
        \cmidrule{2-3}
         & \makecell{Task Planning} &  \makecell{\citep{sim2023chemos, szymanski2023autonomous}} \\
        
        \midrule
        \multirow{2}{*}{6. Experimental Execution} & \makecell{Machine-to-Machine Interface } &  \makecell{ \citep{yoshikawa2023large} } \\
        \cmidrule{2-3}
         & \makecell{Real-Time Data Monitoring} &  \makecell{} \\
        % \midrule
        \bottomrule
    \end{tabular}
\end{adjustbox}
\end{spacing}
\caption{MatSci-LLM tasks based on the roadmap identified in \Cref{fig:mat-sci-lllm-roadmap}.\label{tab:matscillmtasks}}
%%\vspace{-2.5mm}
\end{table}

% \begin{enumerate}
\textcolor{black}{
\textbf{1. Materials Query:} Materials queries may span diverse user queries, such as, "Suggest potential candidate materials for Li-solid state battery electrolytes". Alternatively, more complex queries may require the MatSci-LLM to generate hypotheses based on presented experimental data, a text document or a combination of multiple such sources. As previously described, hypothesis generation remains an open research problem for MatSci-LLMs and may require interaction with other steps in the roadmap. Thus, materials query refers to the initial stage where the problem identification is performed either manually or through an LLM, presenting a research opportunity for novel, specialized querying methods. Emerging work may also build on top of novel human-machine interfaces for designing complex materials systems \citep{kanarik2023human, vasudevan2022discovering} that enable greater efficiency and faster scientific understanding.}\\
\textcolor{black}{\textbf{2. Data Retrieval:} The second step toward materials discovery is to exploit the existing knowledge from MatSci-LLM internal and external knowledge bases. External knowledge includes databases of diverse materials properties (e.g., composition–structure–properties), unstructured data from text, or images, or a combination thereof that capture diverse aspects of the materials simulation, synthesis and characterization pipeline. The vast amount of publications and knowledge sources makes it non-trivial to extract such information. As such, externalizing the knowledge of MatSci-LLMs could be useful. Recent works by \citet{coxwikicrow} and \citet{buehler2024mechgpt} have shown that intentional use of LLMs has the potential to broaden the availability of useful scientific knowledge by externalizing domain-specific LLM-knowledge in a structured, human-interpretable manner. \citet{coxwikicrow} generated annotations for a database of $>15,000$ protein-codings using robust methods that rely on citations and cross-checking of the generated information against the scientific literature. \citet{buehler2024mechgpt} and \citet{venugopal2024matkg} externalized LLM knowledge in a structured knowledge graph, which can be probed by a scientist to further their understanding and potentially make corrections and adjustments as needed. Future work can build on top of these early approaches leading to more reliable retrieval methods along with creating interpretable MatSci-LLMs.
}\\
\textcolor{black}{
\textbf{3. Materials Design:} Based on the query and retrieved information, MatSci-LLMs may directly generate structures based on CIF files \citep{gruver2023finetuned, flam2023language, antunes2023crystal} or in combination with current graph or point-cloud based generative methods \citep{xie2021crystal, jiao2023crystal, merchant2023scaling}. As shown in \citet{zeni2023mattergen, govindarajan2023learning}, conditional materials generation is a promising approach for designing materials with specific properties, where the properties can also be predicted based on the textual description~\cite{rubungo2023llm}. The rapid progress on generative modeling techniques in adjacent fields such as computer vision, as well as the vast space of unsolved materials problems, such as designing complex real-world systems with multiple structures, provides great opportunities for future research work.
} \\
\textcolor{black}{
\textbf{4. Insilico Evaluation:} Code generation abilities can enable tool-agumented MatSci-LLMs to execute complex simulation workflows to evaluate materials designs. Recent work by \citet{buehler2023generative} shows a possible example of how LLMs can be integrated with relevant tools to perform end-to-end insilico design of polymer materials where an LLM can generate a new molecular compound in SMILES notation and then query different LLM-based agents to perform relevant calculations for the same materials. Further examples in \citet{buehler2023generative} show how the LLM system can also set up the relevant computation environment by installing relevant packages, showing further benefits of end-to-end tool integration. While many of these systems have not yet been tested at large scales, this represents a great step forward in constructing impactful MatSci-LLMs. Whereas recent work provides many reasons to be optimistic about LLMs capabilities to solve concrete in-silico MatSci problems, much published work fails to include negative results outlining current LLM failures. As such, it is important to continue to have broader analysis of LLMs' capabilities for code generation in MatSci similar to \citet{zaki2024mascqa}, which can point to relevant research directions for more robust integration of MatSci-LLMs into materials simulation workflows.
} \\
\textcolor{black}{
\textbf{5. Experiment Planning:} Following insilico evaluation, the next step involves the development of experiment plan to synthesize and characterize the materials. LLMs have shown promise in automating simple laboratory experiments \citep{boiko2023autonomous, bran2023chemcrow}, while adjacent work aims to build necessary infrastructure for autonomous laboratories that perform experiments without human intervention \citep{sim2023chemos, szymanski2023autonomous}. The selection of synthesis and characterization remains highly non-trivial and depends significantly on the material systems, length and time scales, and the properties of interest (see App.~\ref{app.matsyn}). As such, further research is needed to have MatSci-LLMs effectively identify realistic, detailed, and executable experimental procedures informed by the constraints of state-of-the-art technology and user needs. Moreover, the development of effective digital twins for different synthesis procedures will be immensely valuable for insilico testing and refinement of experimental plans. Data mining approaches sometimes provide useful directions for targeted use cases, but still require large amount of expert intervention, making them unsuitable for large-scale use. 
} \\
\textcolor{black}{
\textbf{6. Experiment Execution:} The actual execution of the experiments require identification of the relevant commands and the sequence in which these should be given. This also involves intermediate analysis and appropriate modification of the protocol according to the real experimental conditions at a given time. For instance, melting of a silicate system would require continuous strirring until the system is bubble free; a standard protocol while preparing glasses. Thus, MatSci-LLMs should be able to make and change the plans dynamically as per the actual conditions of the experiment. Recent work by \citet{yoshikawa2023large} shows that LLMs can provide practical interfaces that more effectively connect scientists to robotic systems to perform chemical tasks. Current capabilities, however, are still in their early stages with significant future work needed to create robust control methods for a single machine, as well as machine-to-machine communication capabilities.
% \end{enumerate}
}

% In particular, we believe that MatSci-LLMs have the potential to enable three breakthrough capabilities: 1. Augmenting MatSci knowledge with automated knowledge base generation that enhances human understanding; 2. Automated \textit{in-silico} materials design with AI-enabled materials generation and high-fidelity simulations; 3. Self-driving laboratories for materials synthesis and characterization in the real world.

% \subsection{Automated Knowledge Base Generation}

% Recent work by \citet{coxwikicrow} and \citet{buehler2024mechgpt} have shown that intentional use of LLMs has the potential to broaden the availability of useful scientific knowledge by externalizing the knowledge of domain-specific LLMs as structured, human-interpretable knowledge. \citet{coxwikicrow} generated annotations for a database of $>15,000$ protein-coding by using robust methods that rely on citations and cross-checking of the generated information against the scientific literature. \citet{buehler2024mechgpt} externalized LLM knowledge in a structured knowledge graph, which can be probed by a scientist to further their understanding and potentially make corrections and adjustments as needed. Taken together and expanded to related fields, these knowledge bases then become valuable resources for vast sets of engineering applications, spanning the diverse field of MatSci and technology.

% Having interpretable structured knowledge would also allow scientist to make targeted corrections based on their domain expertise.
% One potentially impactful way to test the reliability and robustness of LLM-based generation is to do the generation of interpretable structured language that can consolidate fragemnted knowledge and potentially even augment it. Recent work by \citet{coxwikicrow} and \citet{buehler2024mechgpt} show that intentional use LLMs has the potential to broaden the availability of useful scientific knowledge by externalizing the knowledge of domain-specific LLMs combined with robust methods. Having interpretable structured knowledge would also allow scientist to make targeted corrections based on their domain expertise.



% \subsection{Automated In-Silico Materials Design}

% One of the areas of greatest potential impact for MatSci-LLMs is their ability to provide interfaces between humans and machines. Given the usability of natural language as a human-friendly interface and the ability of LLMs to understand, process and generate text in various formats, including computer code, there is a tremendous opportunity to streamline complex scientific processes. Using code generation, tool-agumented MatSci-LLMs can aid in the discovery of new materials and execution complex simulation workflows. Recent work by \citet{buehler2023generative} shows a possible example of how LLMs can be integrated with relevant tools to perform end-to-end insilico design of polymer materials where the LLM can generate a new molecular compound in SMILES notation and then query different LLM-based agents to perform relevant calculations for the same materials. Further examples in \citet{buehler2023generative} show how the LLM system can also set up the relevant computation environment by installing relevant packages, showing further benefits of end-to-end tool integration. While many of these systems have not yet been tested at large scales, this represents a great step forward in constructing impactful MatSci-LLMs. In addition to code generation, MatSci-LLMs can also serve as generative models for new materials  \citep{flam2023language, gruver2023fine} that augment current graph or point-cloud based representations \citep{xie2021crystal, jiao2023crystal, govindarajan2023learning, merchant2023scaling, zeni2023mattergen}. As such, MatSci-LLMs can devise new materials solution based on their implicit knowledge in addition to leveraging other generative methods as tools for hypothesis generation. 

% While recent work provides many reasons to be optimistic about LLMs capabilities to solve concrete in-silico MatSci problems, much published work fails to include negative results outlining current LLM failures. As such, it is important to continue to have broader analysis of LLMs' capabilities for code generation in MatSci similar to \citet{zaki2024mascqa}, which can point to relevant research directions for more robust integration of MatSci-LLMs into materials simulation workflows. 

% Concretely, \citet{zaki2024mascqa} performed an analysis on the capability of LLMs to generate codes for MatSci domain reveal that GPT4 (gpt-4-0613) obtains a score of only 71.6\% in code writing. Some of the mistakes made by GPT4-CoT are included in the Appendix \todo{Include codes in Appendix and refer here}. This shows that future work is needed for more robust integration of LLMs into materials simulation workflows.

% Another task in which LLMs are known to do well is code generation. Due to their superior performance in code generation, GPT4 has now adopted an approach to solve numerical problems by generating the equivalent code to solve the problem and then running it \todo{REF}.

% The field of tool-augmented LLMs \citep{li-etal-2023-api} provides a useful framework for integrating diverse sets of MatSci tools into complex workflows for diverse sets of materials design cases. \textcolor{red}{would be good to talk about Langchain and other adjacent tools}


% One of the earliest applications of LLMs was code generation \citep{chen2021evaluating} leading to various product releases, such as Github co-pilot and others that helped computer science developers accelerate their development process. Similar opportunities for acceleration scientific simulations that underlie high-throughput screening in MatSci. The diversity of data formats, simulation hyperparameters and associated language based outputs provide a potentially rich set of data and feedback to make LLMs practical tools in accelerating the execution of simulation workflows. 

% \subsection{Self-Driving Laboratories for Sim2Mat}

% One of the areas of greatest potential impact for LLMs in MatSci is their ability to provide interfaces between humans and machines. Given the usability of natural language as a human-friendly interface and the ability of LLMs to understand, process and generate text in various format, including computer code \citep{chen2021evaluating}, this provides a tremendous opportunity to streamline complex scientific processes. 

% Bringing simulated materials to reality (Sim2Mat) and aligning both the experimental and simulation results is the ultimate goal of end-to-end materials design. To that end, MatSci-LLMs can provide a powerful tool to accelerate the process of designing relevant experiments and accelerating their execution. One encouraging fact is that recent research work has seen greater adoption of human-machine interfaces to accelerate the discovery and synthesis of complex materials systems \citep{kanarik2023human, vasudevan2022discovering}, as well as the development of automated self-driving materials laboratories \citep{sim2023chemos, rupnow2023self}. This provides a great opportunity for MatSci-LLMs to further accelerate the process of materials development by providing a connective tissue between the various machines involved in experimental execution. \citet{sim2023chemos} provides an example of how different machines in a laboratory can be connected by a unified software, which then provides an opportunity for MatSci-LLMs to directly interface between machines by translating between distinct software languages required for machine-machine interfaces. Additionally, MatSci-LLMs can provide a language-based interface to human scientists who can define design requirements using natural language similar to \citet{bran2023chemcrow, boiko2023autonomous}, where experimental workflows are executed by tool-augmented LLMs. Recent work by \citet{yoshikawa2023large} also shows that LLMs can provide practical interfaces that more effectively connect scientists to robotic systems to perform chemical tasks. As shown in \Cref{fig:mat-sci-lllm-roadmap}, the ability of MatSci-LLMs to execute experimental workflows has the potential to fully close the loop of the materials discovery cycle providing end-to-end automation of materials design \textit{in-silico}, followed by automated synthesis with recipes that are both human readable and machine executable to bring the desired material into the real-world, finalized by analysis and characterization which also involves machine-to-machine and human-to-machine interactions. 



% \textcolor{black}{
% The challenges and opportunties are -> This is where we want LLMs to go:
% \begin{itemize}
%     \item Tool-augmented LLMs like \citep{bran2023chemcrow, boiko2023autonomous}
%     \item Talk about LLM as code-generation tools for simulation packages
%     \item LLMs for populating knowledge like WikiCrow and HoneyBee
%     \item Synthesis recipe and literature search (can cite example's from Elsa's work here)
% \end{itemize}
% }

==> 6_future_work.tex <==
%\vspace{-0.3cm}
\section{Conclusions and outlook}
%\vspace{-0.2cm}
% Putting together all the parts of MatSci-LLM creates a virtuous cycle for materials discovery shown in \Cref{fig:mat-sci-lllm-roadmap} where scientific automation (machine-to-machine) and scientist-machine augmentation occurs for various of the materials discovery process. 
The virtuous cycle shown in \Cref{fig:mat-sci-lllm-roadmap} has the potential to enable impactful scientific discoveries through end-to-end automation while concurrently augmenting human knowledge through the discovery of new physical and chemical relationships for an expanding set of materials. The unique challenges of deploying LLMs in MatSci outlined in this paper, however, require further research to make MatSci-LLMs effective scientific assistants. 
% MatSci is a diverse field with unique challenges that requires further research work for LLMs to become effective scientific assistants. 
Meaningful research advances will require advances along the interface of many fields, including machine learning, materials simulation, materials synthesis, materials characterization, and robotics. 

% \textcolor{red}{General Workflow: User query - pull from knowledge base - generate hypothesis - run insilico workflow - run experiment workflow - validate hypethesis; Scientific NLP - Materials Simulation/Insilico Design - Self Driving Lab; this is what we envision as the high throughput materials discovery framework - raodmap/this is what we should work towards}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{icml2024/figures/matsci-llm-roadmap-2.png}
%     % %\vspace{-0.3cm}
%     \caption{Roadmap of a Mat-Sci LLM based materials discovery cycle. The cycle starts with materials query from a researcher that specifies desired properties or an application. The MatSci-LLM then draws from external and internal knowledge bases to generate a materials design hypothesis which is evaluated in-silico. Next, the MatSci-LLM ingests the in-silico results and prepares an experimental plan to synthesize and characterize the material, after which the MatSci-LLM interfaces with the relevant machines to execute the experimental workflow. The final result is then shown to the user for evaluation and feedback. Each stage can interact with another for refinement and improvement by the MatSci-LLM. }
%     \label{fig:mat-sci-lllm-roadmap}
%     % %\vspace{-0.5cm}
% \end{figure}

Among the 17 sustainable development goals (SDGs) proposed by United Nations, 10 can be achieved or accelerated through materials innovation. The development of an end-to-end framework for accelerating materials discovery can have broader impacts in several domains such as healthcare, agriculture, energy, sustainability, water filtration, and carbon capture, to name a few. Traditional materials discovery remains an extremely slow process often taking a period of 20-30 years from starting a design to final deployment. AI-driven materials discovery has a potential to reduce this cycle to a few years or even months, thereby providing a means to address major societal-scale challenges. Moreover, the availability of cloud computing and web services can make this process extremely efficient and economical leading to democratization of materials discovery. This could reduce the gap between large corporations and small and medium scale industries allowing materials discovery without the availability of large lab facilities and vast R\&D budgets. 
% Altogether, addressing the challenges discussed here to develop an MatSci LLM can have a significant braoder impact on the future of humanity.
While Mat-Sci LLMs have great promise in reducing the cost and democratizing materials discovery, great care must be taken to ensure that MatSci-LLMs and all related technologies be used in an ethical and harm-limiting manner. {As such, we propose the following framework to reduce the risk of potentially harmful deployment of MatSci-LLMs:
\begin{enumerate}
    \item \textbf{Transparency:} Encouraging sharing of models, datasets, and research methodologies to promote transparency, replication, and validation of findings by the broader scientific community is key to ensure risk mitigation. This approach facilitates peer review and enables independent verification of results and claims. Further, maintaining comprehensive logs of data sources, model training processes, and decision-making pathways should be encouraged to ensure accountability and traceability.
    \item \textbf{Risk Assessment:} Developing methodologies for assessing the risks associated with the application of LLMs in MatSci, focusing on both direct impacts (e.g., safety of newly discovered materials) and indirect impacts (e.g., environmental effects of scaled production) is of paramount importance. Further, systems should be established for ongoing monitoring of the outcomes and impacts of materials discovered or optimized through LLMs to identify and address unforeseen risks promptly.
    \item \textbf{Regulatory Compliance \& Standardization: }Guidelines that address the unique challenges and risks associated with using LLMs in materials discovery should be created and enforced by governing agencies. Furthermore, standards should be developed for data representation, algorithms, and model transparency to facilitate oversight and ensure quality and reliability.
    \item \textbf{Education \& Training: }Education and training programs that integrate ethics, environmental science, sustainability, and AI should be developed to prepare a workforce capable of navigating the complexities of using LLMs in materials discovery. Additionally, dialogues and knowledge exchange between scientists, policymakers, industry stakeholders, and the public to build understanding and trust in AI-driven materials discovery should be facilitated. A noteworthy aspect that requires discussion is the tendency of LLMs to hallucinate. It is important to educate the issues associated with hallucinations in LLMs and how this can have impact on the task that it is applied for.
\end{enumerate}}

One example where MatSci-LLMs could cause unintended harmful consequences relates to the use of natural resources. One can imagine a case where new materials discoveries could put greater demand on minerals that were previously unterutilized. This, in turn, could result in significant impacts on the local communities and the surrounding ecosystem and would therefore require action at policy level to avoid inadvertent consequences.  
